Multimodal Chain-of-Thought Reasoning in Language Models

Large language models (LLMs) have shown impressive performance on complex reasoning by leveraging chain-of-thought (CoT) prompting to generate intermediate reasoning chains as the rationale to infer the answer. However, existing CoT studies have primarily focused on the language modality. We propose Multimodal-CoT that incorporates language (text) and vision (images) modalities into a two-stage framework that separates rationale generation and answer inference. In this way, answer inference can leverage better generated rationales that are based on multimodal information. Experimental results on ScienceQA and A-OKVQA benchmark datasets show the effectiveness of our proposed approach. With Multimodal-CoT, our model under 1 billion parameters achieves state-of-the-art performance on the ScienceQA benchmark. Our analysis indicates that Multimodal-CoT offers the advantages of mitigating hallucination and enhancing convergence speed. Code is publicly available at https://github.com/amazon-science/mm-cot.

==> algorithms/mm-cot-alg.tex <==
\begin{algorithm}[t]\small
    \caption{Multimodal-CoT}\label{alg:mm-cot}
    \begin{algorithmic}[1]
    \Require Language input $X_{\textrm{language}}^{1}$, vision input $X_{\textrm{vision}}$
    \Ensure Generated rationale $R$, inferred answer $A$
    \State Construct the input $X=\{X_{\textrm{language}}, X_{\textrm{vision}}\}$
    \State Generate rationale ${R} = F(X)$ using the model $F(\cdot)$
    % \State Transform sentence-image pair to topic-image lookup table $\mathcal{Q}$ = LookUp($S$, $E$, $\mathcal{F}$)
    \State Append the rationale $R$ to the original language input $X_{\textrm{language}}^{2} = X_{\textrm{language}}^{1} \circ {R}$.
    \State Construct new input $X'=\{X_{\textrm{language}}^{2}, X_{\textrm{vision}}\}$
    \State Infer the answer $A$ by conditioning on the new input, ${A} = F(X')$. 
    \Procedure{F}{$X$}
    \State Encode the language and vision inputs $H_{\textrm{language}}$ and $H_{\textrm{vision}}$, respectively 
    \State Build the interaction between language and vision features by attention $H_{\textrm{vision}}^\textrm{attn}$
    \State Fuse $H_{\textrm{language}}$ and $H_{\textrm{vision}}^\textrm{attn}$ by a gated fusion mechanism to have $H_{\textrm{fuse}}$
    \State Feed $H_{\textrm{fuse}}$ to the decoder to obtain the target prediction $Y$
    \State \textbf{return} $Y$
    \EndProcedure%
    \end{algorithmic}
    
\end{algorithm}
% \vspace{-3mm}
